Wasserstein Distributionally Robust Multiclass Support Vector Machine

We study the problem of multiclass classification for settings where data features $\mathbf{x}$ and their labels $\mathbf{y}$ are uncertain. We identify that distributionally robust one-vs-all (OVA) classifiers often struggle in settings with imbalanced data. To address this issue, we use Wasserstein distributionally robust optimization to develop a robust version of the multiclass support vector machine (SVM) characterized by the Crammer-Singer (CS) loss. First, we prove that the CS loss is bounded from above by a Lipschitz continuous function for all $\mathbf{x} \in \mathcal{X}$ and $\mathbf{y} \in \mathcal{Y}$, then we exploit strong duality results to express the dual of the worst-case risk problem, and we show that the worst-case risk minimization problem admits a tractable convex reformulation due to the regularity of the CS loss. Moreover, we develop a kernel version of our proposed model to account for nonlinear class separation, and we show that it admits a tractable convex upper bound. We also propose a projected subgradient method algorithm for a special case of our proposed linear model to improve scalability. Our numerical experiments demonstrate that our model outperforms state-of-the art OVA models in settings where the training data is highly imbalanced. We also show through experiments on popular real-world datasets that our proposed model often outperforms its regularized counterpart as the first accounts for uncertain labels unlike the latter.

==> Sections/7_checklist.tex <==
\section{Reproducibility Checklist}
This paper:

\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced \hl{YES}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \hl{YES}
\item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \hl{YES}
\item Does this paper make theoretical contributions? \hl{YES}

\begin{enumerate}
\item All assumptions and restrictions are stated clearly and formally. \hl{YES}
\item All novel claims are stated formally (e.g., in theorem statements). \hl{YES}
\item Proofs of all novel claims are included. \hl{YES}
\item Proof sketches or intuitions are given for complex and/or novel results. \hl{YES}
\item Appropriate citations to theoretical tools used are given. \hl{YES}
\item All theoretical claims are demonstrated empirically to hold. \hl{YES}
\item All experimental code used to eliminate or disprove claims is included. \hl{NA}
\item Does this paper rely on one or more datasets? \hl{YES}

\begin{enumerate}
\item A motivation is given for why the experiments are conducted on the selected datasets \hl{YES}
\item All novel datasets introduced in this paper are included in a data appendix. \hl{NA}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \hl{NA}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \hl{YES}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \hl{YES}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \hl{NA}
\item Does this paper include computational experiments? \hl{YES}

\begin{enumerate}
\item Any code required for pre-processing data is included in the appendix. \hl{YES}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. \hl{YES}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \hl{YES}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \hl{YES}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \hl{NA}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \hl{YES}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \hl{YES}
\item This paper states the number of algorithm runs used to compute each reported result. \hl{YES}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \hl{YES}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \hl{NO}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \hl{YES}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \hl{YES}
\end{enumerate}
\end{enumerate}
\end{enumerate}
\end{itemize}
